Cognitive Graph for Multi-Hop Reading Comprehension at Scale

We propose a new CogQA framework for multi-hop question answering in web-scale documents. Inspired by the dual process theory in cognitive science, the framework gradually builds a \textit{cognitive graph} in an iterative process by coordinating an implicit extraction module (System 1) and an explicit reasoning module (System 2). While giving accurate answers, our framework further provides explainable reasoning paths. Specifically, our implementation based on BERT and graph neural network efficiently handles millions of documents for multi-hop reasoning questions in the HotpotQA fullwiki dataset, achieving a winning joint $F_1$ score of 34.9 on the leaderboard, compared to 23.6 of the best competitor.

==> 1.introduction.other.tex <==
Recently,  state-of-the-art  models~\citep{wang2018multi,devlin2018bert} achieve or even outperform human-like performances on various NLP tasks,
including reading comprehension on SQuAD benchmark~\citep{rajpurkar2016squad}, thanks to the large corpus, super computation power, as well as the advanced neural network architectures ~\citep{vaswani2017attention,devlin2018bert}. However, these models are still not sufficient to do complex reasoning, which is required in more practical tasks~\citep{kovcisky2018narrativeqa, jia2017adversarial}. Adversarial tests~\citep{jia2017adversarial} reveal that current models depend on ``advanced pattern matching'' and tend to seek answers near statements similar to the question, leading to failures in complex questions that need multi-hop reasoning.
Several latest datasets are then designed and released, e.g., WikiHop~\citep{welbl2018wikihop}, TriviaQA~\citep{joshi2017triviaqa}, HotpotQA~\citep{yang2018hotpotqa}, among several others, advocating more attention on the true reasoning ability of the learning model. These datasets require searching and reasoning over multiple supporting documents to answer the questions.  

%providing more complex reading comprehension tasks. Unlike the single paragraph QA, these datasets need cross documents or paragraphs reasoning that involves multiple supporting facts or reasoning paths. 
%This show that the current models could be far less powerful than human in reasoning.
%Without explicit reasoning paths, these models can hardly solve complex questions which need iterative reasoning and searching in web-scale documents, far less powerful than human's ability to utilize the memory.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/cg.pdf}
    \caption{An example of cognitive graph. Each \textit{hop node} corresponds to an entity, for example ``Los Angeles''. Each entity has an introductory paragraph. The dashed box means \textit{ans node}, an answer candidate to the question. Cognitive graph mimics human reasoning process. Edges are built when calling an entity to mind. The solid black edges are the correct reasoning path.}
    \label{fig:example}
\end{figure}

%An important development of the social cognitive neuroscience is the so called dual-process and dual-system theory. Particularly interesting is the identification of reflexive (System 1) and reflective (System 2) cognitive processing, with two neurological systems described~\cite{evans1984heuristic,evans2003two,evans2008dualreview,sloman1996empirical}. To be more specific, our brain first retrieves relevant information via an \textit{implicit}, \textit{unconscious} and \textit{uncontrollable} process (System 1), based on which another \textit{explicit}, \textit{conscious} and \textit{controllable} reasoning process is then conducted (System 2). System 2 enables diving deeper into the complex relational structures among the retrieved arguments by performing sequential thinking in a working memory with limited capacity, however slower but with greater evolutionary plausibility~\citep{baddeley1992working}. 
Human beings, though cannot achieve the same efficiency in retrieving related paragraphs for a question, show more comprehensive skills at doing complex reasoning. Revisiting the cognitive process of our thinking, the \emph{dual process theory}~\cite{evans1984heuristic,evans2003two,evans2008dualreview,sloman1996empirical} suggests that our brains first retrieve relevant information via an \textit{implicit}, \textit{unconscious} and \textit{uncontrollable} process (``System 1"), based on which another \textit{explicit}, \textit{conscious} and \textit{controllable} reasoning process is then conducted (``System 2"). System 2 enables diving deeper the complex relational structures among the retrieved arguments by performing sequential thinking in a working memory with limited capacity, slower but with greater evolutionary plausibility~\citep{baddeley1992working}. 
%State-of-the-art models in reading comprehension are really good at retrieving related answers implicitly or unconsciously. Like System 1, these models can work independently or even with the absence of System 2, but they only becomes accurate to give both efficient and reliable conclusions in areas where enough data or exercises are taken. 
Considering the superior power of state-of-art models in implicit answer retrieval, we assume that the reasoning ability may come at the presence of System 2, which explicitly controls the whole reasoning process. 
%The former is also required to be explainable and communicable so that people can be taught and trained by detailed instructions. 

%The gap between the thinking mechanism of human beings and the current end-to-end neural models under the dual process theory, we believe is the ability to explicit control the whole reasoning process, which is also required to be explainable and communicable so that people can be taught and trained by detailed instructions. 
%Current models either focus on discovering implicit distributions in the data ~\citep{blackboxmodels} or designing explicit heuristics~\citep{fuhaoKBheuristic}.
%Evidence can be found in multi-hop reading comprehension tasks.the search space grows exponentially as the answering depth grows.
%The unconscious retrieval process in System 1 can be trained to be both efficient and reliable through enough data or exercises.

%What makes a complex reading comprehension or question answering task ``complex", is that similar Question-Answer structures are insufficient in the training data. It's too difficult for a single model to consider all the possible relationships in a large candidate sets.  

%The missing or misplacing of System 2 results in pool performance in the reasoning tasks.  
%Though system 1 can work independently from System 2, it only becomes accurate to give efficient and reliable conclusions in areas where enough data or exercises have been taken, which is similar in the current models that need exhausted supervision to produce good results. When new questions is issued, we need system 2 to correct belief-bias ~\citep{beliefbias} or create new facts.
%The former process is called ``System 1', whose black-box behavior is quite similar with the current end-to-end models. The later process called ``System 2'' does the reasoning based on the relationships among limited facts retrieved from System 1. 
%The two System 1 alone may lead to a problem called ``belief-bias''~\citep{beliefbias} when System 2 is overwhelmed by distractor tasks~\citep{neys2006dual}.
%Belief bias is the conflicts between logical reasoning and prior knowledge about the ground truth conclusions.
%Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases which is closely related to the defects of current SOTA models in reading comprehension. 
% belief-bias: conflict between logical reasoning and prior knowledge about the truth of conclusions
%Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases. 

%This reasoning skill is taught and trained in a more interpretable and communicatable way, compared to the retrieval skill whose mechanism is much harder to describe. 

% Without explicit reasoning paths,  these models can hardly solve complex questions which need iterative reasoning and searching in web-scale documents, far less powerful than human's ability to utilize the memory.



%To make machines understand natural languages like human has always been a dream for NLP researchers. Recently, the task of reading comprehension and question answering~\citep{rajpurkar2016squad,yang2018hotpotqa} becomes a touchstone of the ability to understand language. 



%(Psychologists suggest that human beings follow a dual process in thinking, where system 1 is an implicit or unconscious process and system 2 is explicit or conscious process. Though System 1 can also give conclusions  independently, it only becomes accurate to give efficient and reliable conclusions in areas where enough data or exercises have been taken . Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases. Inspired by the dual process theory, we propose a dual process framework to tackle tasks and achieve certain explainability. )


%For human beings, the reasoning skill can be taught and trained in a more interpretable and communicatable way, compared to the retrieval skill whose mechanism is much harder to describe. 

% Knowledge Graph has achieved outstanding success in Information retrieval. Unsatisfying at barely retrieve known knowledge, researchers are turning their attention to new knowledge reasoning or knowledge graph completion nowadays~\cite{bordes2013translating}.

% However, traditional knowledge graph only records direct relations, leading it hard to reason out new knowledge. Previous approaches to conquer this problem generally fall into two categories: \emph{embedding based} and \emph{path based}. TransE~\cite{bordes2013translating} and its extensions embed each node in knowledge graph into feature space and preserve the \emph{head-relation-tail} equation. DeepPath~\cite{xiong2017deeppath} however assumes that there is a high-likelihood path in knowledge graph from the head node to the tail node.

%When revisiting cognition process of human brain, we find that we do not conclude based on matching question with relevant statements. Our brain first pays attention to key entities when reading, synthesizes their semantics. This process is called ``System 1'' according to \emph{dual process theory} in cognition science, which . Then ``System 2'' does reasoning based on retrieved knowledge and explicit relations in working memory at a further level of granularity~\citep{rumelhart1986parallel}.


% In this paper, we present a framework \emph{cognitive graph} for natural language comprehension and question answering which consists of two functionally different systems, according to the dual process theory. System 1 is responsible for synthesizing out the semantics of only a few question-relevant entity arguments extracted from paragraphs into the working memo‘ry of System 2. System 2 only considers the nodes  produced by System 1 in its working memory, constructs a corresponding cognitive graph and conducts the reasoning tasks with explicit reasoning path, thus being highly explainable. We also allow back-and-forth process between System 1 and System 2 to expand the candidate answers on demand. The process is also highly scalable to tackle QA tasks over web-scale documents that our implementation using BERT and Graph Neural Network can efficiently train and evaluate on a full wiki(>5,000,000 documents) Multi-Hop QA datasets, with a substantial improvement on all the metrics over the best results on the leaderboard.

%In addition to relation edges, knowledge is organized into abstract concepts in a hierarchical way. When doing reasoning, we continue visiting high-level concept nodes, which both predict useful concept nodes and generate instance nodes into a small \emph{thought graph}. Analogous to working memory in human brain, thought graphs contains knowledge nodes related to the question and produce final results by leveraging Graph Neural Networks~\citep{battaglia2018relational}.
In this paper, we propose a framework, namely \emph{Cognitive Graph QA}(\name), consisting of two functionally different systems for natural language comprehension and question answering (QA), inspired by the dual process theory. 
%The framework builds a cognitive graph of entities iteratively by coordinating the two systems. System 1 receives some reasoning clues produced by System 2 in the previous step, and predicts the next hop nodes or answer nodes in the . System 2 .
%System 1 only tries to extract the semantic information on the entity
System 1 extracts question-relevant entities and answer candidates from paragraphs and encodes their semantic information. Extracted entities are organized as a relational \emph{cognitive graph}(Figure~\ref{fig:example}), which resembles the working memory for deeper reasoning in System 2. System 2 then conducts the reasoning procedure over the graph, and collects \textit{clues} to guide System 1 to better extract next-hop entities. The above process is iterated until all possible answers are found, and then the final answer is chosen based on all processed information.

\emph{Cognitive graph} explains reasoning process visually at entity level and is highly scalable to tackle QA tasks over web-scale documents. 
 % According to the CGP framework,
 Meanwhile, our implementation using BERT~\cite{devlin2018bert} and Graph Neural Network (GNN)\cite{battaglia2018relational} efficiently handles fullwiki-wide with more than five million documents for the multi-hop reasoning questions in the HotpotQA~\citep{yang2018hotpotqa} dataset, with a substantial improvement on all the metrics over the best competitors.

%\zc{\textbf{Challenge Materials.} This part is used as a temporary challenge center.Why existing methods fail in multi-hop QA?The definition of Multi-Hop QA. Imagine that each paragraph in the corpus describes a relation between two entities (ignore super node and relation first). All these relations can be generated from a least information graph, in which any removal of the graph edge will result in inconsistency conclusion with the corpus. Any question in current QA tasks corresponds to a specific subgraph, where entities and relations about that question can be inferred from the least information graph. So it's trivial that the performance of QA models are related to the ability to infer unseen relations using the least information graph.We factorize the ability. If there is enough redundancy or shortcut edges in the corpus graph that overlaps with the question set, in this case, one hop semantic match will do the job.Question hop and answer hop. We also consider question $Q$ as least information question without redundancy that the removal of any relation or entity will result in an inconsistent answer. $Q_hop$ describes a question can be formed as a single relation problem, }

==> 1.introduction.tex <==
Recently,  state-of-the-art  models~\citep{wang2018multi,devlin2018bert} achieve or even outperform human-like performances on various NLP tasks,
including reading comprehension on the Stanford Question Answering Dataset (SQuAD) benchmark~\citep{rajpurkar2016squad}, thanks to the large corpus, super computation power, as well as the advanced neural network architectures ~\citep{vaswani2017attention,devlin2018bert}. However, these models are still not sufficient to do complex reasoning, which is required in more practical tasks~\citep{kovcisky2018narrativeqa, jia2017adversarial}. Adversarial tests~\citep{jia2017adversarial} further demonstrate that no published open-source model is robust to the addition of adversarial sentences due to the fact that existing models are overly stable to perturbations that alter semantics. Thus they are usually unable to answer complex questions that need dedicated reasoning or multi-hop searching.
Several latest datasets are then designed and  released, e.g., WikiHop~\citep{welbl2018wikihop}, TriviaQA~\citep{joshi2017triviaqa}, HotpotQA~\citep{yang2018hotpotqa}, among several others, to advocate more attention on the true reasoning ability of the learning model by requiring searching and reasoning over multiple supporting documents to answer diverse questions that are not constrained to any pre-existing knowledge bases or knowledge schemas. 
%providing more complex reading comprehension tasks. Unlike the single paragraph QA, these datasets need cross documents or paragraphs reasoning that involves multiple supporting facts or reasoning paths. 
%This show that the current models could be far less powerful than human in reasoning.
%Without explicit reasoning paths, these models can hardly solve complex questions which need iterative reasoning and searching in web-scale documents, far less powerful than human's ability to utilize the memory.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/cg.pdf}
    \caption{An example of cognitive graph for multi-hop QA. Each \textit{hop node} corresponds to an entity following by its introductory paragraph, for example ``Los Angeles''. The circles mean \textit{ans nodes}, answer candidates to the question. Cognitive graph mimics human reasoning process. Edges are built when calling an entity to mind. The solid black edges are the correct reasoning path.}
    \label{fig:example}
\end{figure}
An important development of the social cognitive neuroscience is the so called dual-process and dual-system theory. Particularly interesting is the identification of reflexive (System 1) and reflective (System 2) cognitive processing, with two neurological systems described~\cite{evans1984heuristic,evans2003two,evans2008dualreview,sloman1996empirical}. To be more specific, our brain first retrieves relevant information via an \textit{implicit}, \textit{unconscious} and \textit{uncontrollable} process (System 1), based on which another \textit{explicit}, \textit{conscious} and \textit{controllable} reasoning process is then conducted (System 2). System 2 enables diving deeper into the complex relational structures among the retrieved arguments by performing sequential thinking in a working memory with limited capacity, however slower but with greater evolutionary plausibility~\citep{baddeley1992working}. 
%Human beings, though cannot achieve the same efficiency in retrieving large amount of exact matches for a question, show more comprehensive skills at doing complex reasoning. Revisiting the cognitive process of our thinking, the \emph{dual process theory}~\cite{evans1984heuristic,evans2003two,evans2008dualreview,sloman1996empirical} suggest that our brain first retrieve relevant information via an \textit{implicit}, \textbf{unconscious} and \textbf{uncontrollable} process (``System 1"), based on which another \textbf{explicit}, \textbf{conscious} and \textbf{controllable} reasoning process is then conducted (``System 2"). System 2 enables diving deeper the complex relational structures among the retrieved arguments by performing sequential thinking in a working memory with limited capacity, which is much slower~\citep{workingmem}. 
%State-of-the-art models in reading comprehension are really good at retrieving related answers implicitly or unconsciously. Like System 1, these models can work independently or even with the absence of System 2, but they only becomes accurate to give both efficient and reliable conclusions in areas where enough data or exercises are taken. 
We assume that the gap between the thinking mechanism of human beings and the current end-to-end neural models under the dual process is the ability to explicitly control the whole reasoning process. The former is also required to be explainable and communicable so that people can be taught and trained by detailed instructions. 

%The gap between the thinking mechanism of human beings and the current end-to-end neural models under the dual process theory, we believe is the ability to explicit control the whole reasoning process, which is also required to be explainable and communicable so that people can be taught and trained by detailed instructions. 
%Current models either focus on discovering implicit distributions in the data ~\citep{blackboxmodels} or designing explicit heuristics~\citep{fuhaoKBheuristic}.
%Evidence can be found in multi-hop reading comprehension tasks.the search space grows exponentially as the answering depth grows.
%The unconscious retrieval process in System 1 can be trained to be both efficient and reliable through enough data or exercises.

%What makes a complex reading comprehension or question answering task ``complex", is that similar Question-Answer structures are insufficient in the training data. It's too difficult for a single model to consider all the possible relationships in a large candidate sets.  

%The missing or misplacing of System 2 results in pool performance in the reasoning tasks.  
%Though system 1 can work independently from System 2, it only becomes accurate to give efficient and reliable conclusions in areas where enough data or exercises have been taken, which is similar in the current models that need exhausted supervision to produce good results. When new questions is issued, we need system 2 to correct belief-bias ~\citep{beliefbias} or create new facts.
%The former process is called ``System 1', whose black-box behavior is quite similar with the current end-to-end models. The later process called ``System 2'' does the reasoning based on the relationships among limited facts retrieved from System 1. 
%The two System 1 alone may lead to a problem called ``belief-bias''~\citep{beliefbias} when System 2 is overwhelmed by distractor tasks~\citep{neys2006dual}.
%Belief bias is the conflicts between logical reasoning and prior knowledge about the ground truth conclusions.
%Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases which is closely related to the defects of current SOTA models in reading comprehension. 
% belief-bias: conflict between logical reasoning and prior knowledge about the truth of conclusions
%Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases. 

%This reasoning skill is taught and trained in a more interpretable and communicatable way, compared to the retrieval skill whose mechanism is much harder to describe. 

% Without explicit reasoning paths,  these models can hardly solve complex questions which need iterative reasoning and searching in web-scale documents, far less powerful than human's ability to utilize the memory.



%To make machines understand natural languages like human has always been a dream for NLP researchers. Recently, the task of reading comprehension and question answering~\citep{rajpurkar2016squad,yang2018hotpotqa} becomes a touchstone of the ability to understand language. 



%(Psychologists suggest that human beings follow a dual process in thinking, where system 1 is an implicit or unconscious process and system 2 is explicit or conscious process. Though System 1 can also give conclusions  independently, it only becomes accurate to give efficient and reliable conclusions in areas where enough data or exercises have been taken . Belief-bias will emerge that the performance drops as the capacity of the working memory in system 2 decreases. Inspired by the dual process theory, we propose a dual process framework to tackle tasks and achieve certain explainability. )


%For human beings, the reasoning skill can be taught and trained in a more interpretable and communicatable way, compared to the retrieval skill whose mechanism is much harder to describe. 

% Knowledge Graph has achieved outstanding success in Information retrieval. Unsatisfying at barely retrieve known knowledge, researchers are turning their attention to new knowledge reasoning or knowledge graph completion nowadays~\cite{bordes2013translating}.

% However, traditional knowledge graph only records direct relations, leading it hard to reason out new knowledge. Previous approaches to conquer this problem generally fall into two categories: \emph{embedding based} and \emph{path based}. TransE~\cite{bordes2013translating} and its extensions embed each node in knowledge graph into feature space and preserve the \emph{head-relation-tail} equation. DeepPath~\cite{xiong2017deeppath} however assumes that there is a high-likelihood path in knowledge graph from the head node to the tail node.

%When revisiting cognition process of human brain, we find that we do not conclude based on matching question with relevant statements. Our brain first pays attention to key entities when reading, synthesizes their semantics. This process is called ``System 1'' according to \emph{dual process theory} in cognition science, which . Then ``System 2'' does reasoning based on retrieved knowledge and explicit relations in working memory at a further level of granularity~\citep{rumelhart1986parallel}.


% In this paper, we present a framework \emph{cognitive graph} for natural language comprehension and question answering which consists of two functionally different systems, according to the dual process theory. System 1 is responsible for synthesizing out the semantics of only a few question-relevant entity arguments extracted from paragraphs into the working memo‘ry of System 2. System 2 only considers the nodes  produced by System 1 in its working memory, constructs a corresponding cognitive graph and conducts the reasoning tasks with explicit reasoning path, thus being highly explainable. We also allow back-and-forth process between System 1 and System 2 to expand the candidate answers on demand. The process is also highly scalable to tackle QA tasks over web-scale documents that our implementation using BERT and Graph Neural Network can efficiently train and evaluate on a full wiki(>5,000,000 documents) Multi-Hop QA datasets, with a substantial improvement on all the metrics over the best results on the leaderboard.

%In addition to relation edges, knowledge is organized into abstract concepts in a hierarchical way. When doing reasoning, we continue visiting high-level concept nodes, which both predict useful concept nodes and generate instance nodes into a small \emph{thought graph}. Analogous to working memory in human brain, thought graphs contains knowledge nodes related to the question and produce final results by leveraging Graph Neural Networks~\citep{battaglia2018relational}.
To fill the above gap, we propose a framework, namely \emph{cognitive graph QA}(\name), consisting of two functionally different systems for natural language comprehension and question answering (QA). System 1 extracts question-relevant entities and answer candidates from paragraphs and encodes their semantic information. Extractions are organized as a relational \emph{cognitive graph}(Figure~\ref{fig:example}), which resembles working memory in cognition for deeper reasoning in the next stage. In System 2, the semantic information is processed during the propagation along explicit reasoning paths. As a response, System 2 collects \textit{clues} to guide System 1 to better extract next-hop entities to expand the graph to answer the specific question. The above process is iterated until all possible answers are found, and then the final answer is chosen based on all processed information.

\emph{Cognitive graph} explains reasoning process visually at word level and is highly scalable to tackle QA tasks over web-scale documents. 
 % According to the CGP framework,
 Meanwhile, our implementation using BERT~\cite{devlin2018bert} and Graph Neural Network (GNN)\cite{battaglia2018relational} efficiently handles fullwiki-wide with more than five million documents for the multi-hop reasoning questions in the HotpotQA dataset, with a substantial improvement on all the metrics over the best competitors.

%\zc{\textbf{Challenge Materials.} This part is used as a temporary challenge center.Why existing methods fail in multi-hop QA?The definition of Multi-Hop QA. Imagine that each paragraph in the corpus describes a relation between two entities (ignore super node and relation first). All these relations can be generated from a least information graph, in which any removal of the graph edge will result in inconsistency conclusion with the corpus. Any question in current QA tasks corresponds to a specific subgraph, where entities and relations about that question can be inferred from the least information graph. So it's trivial that the performance of QA models are related to the ability to infer unseen relations using the least information graph.We factorize the ability. If there is enough redundancy or shortcut edges in the corpus graph that overlaps with the question set, in this case, one hop semantic match will do the job.Question hop and answer hop. We also consider question $Q$ as least information question without redundancy that the removal of any relation or entity will result in an inconsistent answer. $Q_hop$ describes a question can be formed as a single relation problem, }

==> 2.framework.old.tex <==
\section{Cognitive Graph QA Framework}\label{frame}
\begin{algorithm}[hbt]
\small
\SetInd{1pt}{7pt}
\caption{Cognitive Graph QA}\label{algo}
\KwIn{
    \\
    System 1 model $\&S_1$, System 2 model $\&S_2$,\\
    Question $Q$, Predictor $\&F$,Wiki Database $\&W$\\
    }
Initialize cognitive graph $\&G$ with entities mentioned in $Q$\\
Initialize the frontier nodes as all nodes in $\&G$\\
\Repeat{there is no frontier node in $\&G$}{
    %select an unvisited node $x$ to visit\\ 
    pop a node $x$ from frontier nodes\\
    locate $para[x]$ in $\&W$\\
    collect $clues[x,\&G]$ from previous nodes of $x$\\
    generate $sem[x,Q,clues]$ with $\&S_1$\\
    \If{$x$ is a hop node}{
        find hop and answer spans in $para[x]$ with $\&S_1$\\
        \For{$y$ in spans}{
            \uIf{$y \in \&G$ and edge$(x,y)\notin \&G$}{add $y$ to frontier nodes}\ElseIf{$y\notin \&G$ and $y \in \&W$}{create a new frontier node for $y$}
              add edge $(x,y)$ to $\&G$
      
        }
    }
    update hidden representation $\mathbf{X}$ with $\&S_2$
}
\textbf{Return} $\argmax\limits_{\text{answer node }x} \&F(\*X[x])$
\end{algorithm}
Inspired by the dual process theory, our cognitive graph QA framework contains an implicit extraction module called System 1 and an explicit reasoning module called System 2. The framework gradually builds a cognitive graph by coordinating the two systems in an iterative process.

\textbf{Cognitive Graph} is the central data structure in the framework that is expanded through an iterative process. Each \textit{node} in cognitive graph corresponds with an entity or possible answer $x$, abbreviated as node $x$. For any \textit{frontier node} $x$ that is newly added or updated in the cognitive graph $\&G$, the framework conducts a reasoning procedure to produce the understanding about $x$ w.r.t $\&G$ and the question $Q$ using system 2, in the form of hidden representation $\mathbf{X}[x]$. 
System 2 then collects clues, denoted by $clues[x,\&G]$, from all the previous nodes of $x$ in $\&G$. These clues could be sentences, hidden representations or other form of information which can afterwards trigger System 1 to find next-hop entities or possible answers, leading to expansion of the cognitive graph for further reasoning.
% next possible hop node or answer node and expand the cognitive graph for further reasoning. 

\textbf{System 1} takes as input the $clues[x,\&G]$ and the paragraph $para[x]$ that describes $x$ from the documents, extracts the semantics of $x$, $sem[x,Q,clues]$ , based on these clues as $sem[x,Q,clues]$ and identifies the next hop node as well as the answer node.

\textbf{System 2} performs comprehensive reasoning over the current cognitive graph, creates or updates the understanding of any node $x$ in $\&G$ as hidden representation $\mathbf{X}[x]$ based on its semantic vector. 
It also collects the $clues[x,\&G]$ for any node $x$ in the graph $\&G$.

Algorithm~\ref{algo} describes how our \name~framework works given any System 1 and System 2 implementations. Each entity is represented by a \textit{node} in cognitive graph $\&G$. We first initialize the graph with entities mentioned in the question, which are extracted by System 1 with empty clues. Then we iteratively visit each frontier node $x$ and locate its document $para[x]$. $\&G$ is expanded with the extracted next-hop entities (hop node) and answer candidates (answer node). A node $x$ should be revisited once acquiring new $clues[x,\&G]$, i.e., when there is a new edge links to it. Finally, a predictor model predicts answer probabilities of candidates based on the final hidden representation $\mathbf{X}$ from System 2.

==> 2.framework.tex <==
\section{Cognitive Graph QA Framework}\label{frame}
\begin{algorithm}[hbt]
\small
\SetInd{1pt}{7pt}
\caption{Cognitive Graph QA}\label{algo}
\KwIn{
    \\
    System 1 model $\&S_1$, System 2 model $\&S_2$,\\
    Question $Q$, Predictor $\&F$,Wiki Database $\&W$\\
    }
Initialize cognitive graph $\&G$ with entities mentioned in $Q$\\
Initialize the frontier nodes as all nodes in $\&G$\\
\Repeat{there is no frontier node in $\&G$}{
    %select an unvisited node $x$ to visit\\ 
    pop a node $x$ from frontier nodes\\
    locate $para[x]$ in $\&W$\\
    collect $clues[x,\&G]$ from previous nodes of $x$\\
    generate $sem[x,Q,clues]$ with $\&S_1$\\
    \If{$x$ is a hop node}{
        find hop and answer spans in $para[x]$ with $\&S_1$\\
        \For{$y$ in spans}{
            \uIf{$y \in \&G$ and edge$(x,y)\notin \&G$}{add $y$ to frontier nodes}\ElseIf{$y\notin \&G$ and $y \in \&W$}{create a new frontier node for $y$}
              add edge $(x,y)$ to $\&G$
      
        }
    }
    update hidden representation $\mathbf{X}$ with $\&S_2$
}
\textbf{Return} $\argmax\limits_{\text{answer node }x} \&F(\*X[x])$
\end{algorithm}
The nature of multi-hop QA is that the reasoning process usually follows a multi-step fashion. 
We human beings, when trying to answer complex multi-hop questions, usually need iterative steps to cooperate two different types of thinking. By understanding the question, we extract the entities,  
search and extract useful arguments about the entities, guided by the question. 
This process is a fast and implicit process which may refer to System 1 in dual process theory.
Then we will conduct complex reasoning process given the limited information that we assume to be related. 
This process is slow, explicit and may refer to System 2, since we need to figure out the complex logic rigor among these arguments and we can explicit tell other people how we come up with the answer. For complex multi-hop questions, a single step may be insufficient. If we are not familiar with the question, we possibly need to find some clues by analyzing the current arguments.
Then the clues will guide the System 1 to search and extract new arguments, to form a closed loop. 
%Existing retrieve-and-extractor framework may work in single paragraph QA but not adequate for multi-hop ones, since extractor in SOTA models are usually black-box thus is hard to cooperate with the retrieval.

To mimic the process of answering multi-hop questions of human beings, our cognitive graph QA framework contains an implicit extraction module called System 1, and an explicit reasoning module called System 2. 
To simulate the working memory where the reasoning process takes place, we propose a data structure, \textit{Cognitive Graph}, which is gradually expanded by coordinating the two systems in an iterative process.

Each \textit{node} in cognitive graph corresponds with an entity or possible answer $x$, abbreviated as node $x$. For any \textit{frontier node} $x$ that is newly added or updated in the cognitive graph $\&G$, the framework conducts a reasoning procedure to produce the understanding about $x$ w.r.t $\&G$ and the question $Q$ using system 2, in the form of hidden representation $\mathbf{X}[x]$. 
System 2 then collects clues, denoted by $clues[x,\&G]$, from all the previous nodes of $x$ in $\&G$. These clues could be sentences, hidden representations or other form of information which can afterwards trigger System 1 to find next-hop entities or possible answers, leading to expansion of the cognitive graph for further reasoning.
% next possible hop node or answer node and expand the cognitive graph for further reasoning. 

\textbf{System 1} takes as input the $clues[x,\&G]$ and the paragraph $para[x]$ that describes $x$ from the documents, extracts the semantics of $x$, $sem[x,Q,clues]$ , based on these clues as $sem[x,Q,clues]$ and identifies the next hop node as well as the answer node.

\textbf{System 2} performs comprehensive reasoning over the current cognitive graph, creates or updates the understanding of any node $x$ in $\&G$ as hidden representation $\mathbf{X}[x]$. 
It also collects the $clues[x,\&G]$ for any node $x$ in the graph $\&G$.

Algorithm~\ref{algo} describes how our \name~framework works given any System 1 and System 2 implementations. 
%We first initialize the graph with entities mentioned in the question, which are extracted by System 1 with empty clues. Then we iteratively visit each frontier node $x$ and locate its document $para[x]$. $\&G$ is expanded with the extracted next-hop entities (hop node) and answer candidates (answer node). A node $x$ should be revisited once acquiring new $clues[x,\&G]$, i.e., when there is a new edge links to it. Finally, a predictor model predicts answer probabilities of candidates based on the final hidden representation $\mathbf{X}$ from System 2.


==> 2.framework.three.tex <==
\section{Cognitive Graph QA Framework}\label{frame}
\begin{algorithm}[hbt]
\small
\SetInd{1pt}{7pt}
\caption{Cognitive Graph QA}\label{algo}
\KwIn{
    \\
    System 1 model $\&S_1$, System 2 model $\&S_2$,\\
    Question $Q$, Predictor $\&F$,Wiki Database $\&W$\\
    }
Initialize cognitive graph $\&G$ with entities mentioned in $Q$\\
Initialize the frontier nodes as all nodes in $\&G$\\
\Repeat{there is no frontier node in $\&G$}{
    %select an unvisited node $x$ to visit\\ 
    pop a node $x$ from frontier nodes\\
    locate $para[x]$ in $\&W$\\
    collect $clues[x,\&G]$ from predecessor nodes of $x$\\
    generate $sem[x,Q,clues]$ with $\&S_1$\\
    \If{$x$ is a hop node}{
        find hop and answer spans in $para[x]$ with $\&S_1$\\
        \For{$y$ in spans}{
            \uIf{$y \in \&G$ and edge$(x,y)\notin \&G$}{add $y$ to frontier nodes}\ElseIf{$y\notin \&G$ and $y \in \&W$}{create a new frontier node for $y$}
              add edge $(x,y)$ to $\&G$
      
        }
    }
    update hidden representation $\mathbf{X}$ with $\&S_2$
}
\textbf{Return} $\argmax\limits_{\text{answer node }x} \&F(\*X[x])$
\end{algorithm}

\name~framework mimics the iterative process of human brains for multi-hop QA, trying to acquire strong reasoning power, entity-level explainability and scalability at the same time.

Our framework relies on a data structure called \textit{cognitive graph} to achieve ordered and entity-level explainability for multi-hop QA. Cognitive graph is a directed graph whose nodes represent entities and edges represent the paragraphs of this linkage, see Figure \ref{fig:example}. Each node is also attached with a semantic vector that represents the current understanding about that node given the question. Compared to other forms of structure, e.g., memory network, whose internal states are completely implicit, cognitive graph is much easier to train since we can build explicit samples for each construction step of the graph and provide higher-quality supervision.
Cognitive graph is also the basis of the reasoning module of System 2, which is responsible to give the final conclusions or the clues for the next step. The construction of the graph, however, is made by the other module, System 1.

The reasoning abilities of \name~framework stem from the System 2. System 2 is responsible for updating the semantic vector, or the understanding, of each node in the cognitive graph given the question. Having these understandings, a predictor model infers which could be the answer of the question. Besides, System 2 also provides clues for System 1, to expand the graph for further reasoning if necessary. This is because for complex questions that we are not familiar with, a single reasoning step is often insufficient to cover those paragraphs that only become semantic-related until some predecessor clues are found. 


System 1 follows an implicit process that is responsible for understanding questions, predicting the next nodes to be considered given the reasoning clues. It also provides the initial semantic vector of each node in the cognitive graph. Advanced deep learning models for QA tasks which outperformed human beings can be applied to implement System 1.

%It's a fast and implicit process which may refer to System 1 in dual process theory.
%It seems to be currently the only part that human tends to lose against the SOTA deep learning models, due to the limited memory capacity and computational power. 

Algorithm~\ref{algo} describes the specific process of our \name~framework given any System 1 and System 2 implementations. 
We first initialize the cognitive graph $\&G$ with entities mentioned in the question. The initial entities are extracted by System 1 with empty clues. Then we iteratively visit each frontier node $x$ and locate its document $para[x]$. 
The clues from all the predecessor nodes of $x$ in $\&G$, denoted by $clues[x,\&G]$, could be sentences, hidden representations or other form of information. 
These clues then trigger System 1 to find next-hop entities or possible answers and extract the semantics of $x$ as $sem[x,Q,clues]$, leading to expansion of $\&G$ for further reasoning. A node $x$ should be revisited once acquiring new $clues[x,\&G]$, i.e., when there is a new edge links to it. Finally, a predictor model predicts answer probabilities of candidates based on the final hidden representation $\mathbf{X}$ from System 2.


==> 2.framework.two.tex <==
\section{Cognitive Graph QA Framework}\label{frame}
\begin{algorithm}[hbt]
\small
\SetInd{1pt}{7pt}
\caption{Cognitive Graph QA}\label{algo}
\KwIn{
    \\
    System 1 model $\&S_1$, System 2 model $\&S_2$,\\
    Question $Q$, Predictor $\&F$,Wiki Database $\&W$\\
    }
Initialize cognitive graph $\&G$ with entities mentioned in $Q$\\
Initialize the frontier nodes as all nodes in $\&G$\\
\Repeat{there is no frontier node in $\&G$}{
    %select an unvisited node $x$ to visit\\ 
    pop a node $x$ from frontier nodes\\
    locate $para[x]$ in $\&W$\\
    collect $clues[x,\&G]$ from predecessor nodes of $x$\\
    generate $sem[x,Q,clues]$ with $\&S_1$\\
    \If{$x$ is a hop node}{
        find hop and answer spans in $para[x]$ with $\&S_1$\\
        \For{$y$ in spans}{
            \uIf{$y \in \&G$ and edge$(x,y)\notin \&G$}{add $y$ to frontier nodes}\ElseIf{$y\notin \&G$ and $y \in \&W$}{create a new frontier node for $y$}
              add edge $(x,y)$ to $\&G$
      
        }
    }
    update hidden representation $\mathbf{X}$ with $\&S_2$
}
\textbf{Return} $\argmax\limits_{\text{answer node }x} \&F(\*X[x])$
\end{algorithm}
%The nature of multi-hop QA is that the reasoning process usually follows a multi-step fashion. 
%Human beings show superior reasoning ability at answering multi-hop questions while achieving entity-level explainability. Our brains  interleave the two different types of thinking iteratively, i.e., collecting puzzles from our memory and reasoning clues at hand.
%The process is also highly scalable that we can answer questions from our memory. 

%Inspired by the dual process theory, 
\name~framework mimics the intuitive process of human brains for multi-hop QA, trying to acquire strong reasoning power, entity-level explainability and scalability at the same time.

%To  part of \name~framework,
%When answering  is teh complex multi-hop questions, we usually need iterative steps to coordinate two different types of thinking. 


%In \name~framework, System 1 is designed to be both scalable and efficient to collect relevant information for further reasoning.

System 1 follows an implicit process that is responsible for understanding questions, predicting the information to be considered, and extracting the semantics of entities given the reasoning clues.
%It's a fast and implicit process which may refer to System 1 in dual process theory.
It seems to be currently the only part that human tends to lose against the SOTA deep learning models, due to the limited memory capacity and computational power. 

To acquire reasoning abilities with entity-level explainability, we design System 2 along with a \textit{cognitive graph} as the structure of working memory. 
%these abilities are achieved through a slow but explicit reasoning process given the limited information collected by System 1. 
Our brains investigate complex logic rigors among the collected information with limited capacity, in a slow but rather explicit way. Explicit here also stands for explainability, which indicates that the reasoning process can be described w.r.t. high-level concept, e.g., entities, text, rules, and can be understood by others.
%The structured information in working memory is referred to as
In \name~framework, \textit{cognitive graph} is a directed graph where each \textit{node} $x$ corresponds with an entity or possible answer. The direct edge $(x,y)$ is a paragraph of $x$ that mentions $y$. System 2 conducts comprehensive reasoning over the cognitive graph, then attaches the result, a hidden representation $\mathbf{X}[x]$ for each node. The cognitive graph captures the explicit relations among the entity nodes thus achieving entity-level explainability. 
%For any \textit{frontier node} $x$ that is newly added or updated in the cognitive graph $\&G$, the framework conducts a reasoning procedure to produce the understanding about $x$ w.r.t $\&G$ and the question $Q$ using system 2, in the form of hidden representation $\mathbf{X}[x]$. System 2 then collects clues, denoted by $clues[x,\&G]$, from all the previous nodes of $x$ in $\&G$. These clues could be sentences, hidden representations or other form of information which can afterwards trigger System 1 to find next-hop entities or possible answers, leading to expansion of the cognitive graph for further reasoning.

%System 1 in dual process theory can work independently, but only becomes efficient and reliable when excessive similar data or exercises are taken. However, 

%For complex questions that we are not familiar with, a multi-step reasoning process is adopted. We interleave the two systems iteratively and construct the cognitive graph step by step, thus providing \textit{ordered} and  \textit{entity-level} explainability.  Like ourselves, we need to find some clues by analyzing the current puzzles in System 2, and continually collect puzzles that needed to proceed the seeking in System 1 with the help of the clues, forming a closed loop. In this iterative process, the cognitive graph in the working memory is gradually expanded by the two systems.


%While System 1 in dual process theory can work properly without System 2 in simple problems, it only becomes efficient and reliable when excessive similar data or exercises are taken.

For complex questions that we are not familiar with, a single reasoning step is often insufficient. Instead, our brains are likely to interleave the two types of thinking iteratively, i.e., finding some clues by reasoning over the current information at hand, and collecting more related information with the help of these clues, forming a closed loop. 
We interleave the two systems in an iterative multi-step reasoning process described in Algorithm \ref{algo},
where the cognitive graph is expanded by the two systems step by step, thus providing \textit{ordered} and \textit{entity-level} explainability.



%Existing retrieve-and-extractor framework may work in single paragraph QA but not adequate for multi-hop ones, since extractor in SOTA models are usually black-box thus is hard to cooperate with the retrieval.




%To mimic the process of answering multi-hop questions of human beings, our cognitive graph QA framework contains an implicit extraction module called System 1, and an explicit reasoning module called System 2. To simulate the working memory where the reasoning process takes place, we propose a data structure, , which is gradually expanded by coordinating the two systems in an iterative process.

%The followings demonstrate the necessary functions of each component in more detail.  

%\textbf{Cognitive Graph} Each \textit{node} in cognitive graph corresponds with an entity or possible answer $x$, abbreviated as node $x$. For any \textit{frontier node} $x$ that is newly added or updated in the cognitive graph $\&G$, the framework conducts a reasoning procedure to produce the understanding about $x$ w.r.t $\&G$ and the question $Q$ using system 2, in the form of hidden representation $\mathbf{X}[x]$. System 2 then collects clues, denoted by $clues[x,\&G]$, from all the previous nodes of $x$ in $\&G$. These clues could be sentences, hidden representations or other form of information which can afterwards trigger System 1 to find next-hop entities or possible answers, leading to expansion of the cognitive graph for further reasoning.
% next possible hop node or answer node and expand the cognitive graph for further reasoning. 

%\textbf{System 1} takes as input the $clues[x,\&G]$ and the paragraph $para[x]$ that describes $x$ from the documents, extracts the semantics of $x$, $sem[x,Q,clues]$ , based on these clues as $sem[x,Q,clues]$ and identifies the next hop node as well as the answer node.

%\textbf{System 2} performs comprehensive reasoning over the current cognitive graph, creates or updates the understanding of any node $x$ in $\&G$ as hidden representation $\mathbf{X}[x]$. It also collects the $clues[x,\&G]$ for any node $x$ in the graph $\&G$.

Algorithm~\ref{algo} describes the specific process of our \name~framework given any System 1 and System 2 implementations. 
We first initialize the cognitive graph $\&G$ with entities mentioned in the question. The initial entities are extracted by System 1 with empty clues. Then we iteratively visit each frontier node $x$ and locate its document $para[x]$. 
The clues from all the predecessor nodes of $x$ in $\&G$, denoted by $clues[x,\&G]$, could be sentences, hidden representations or other form of information. 
These clues then trigger System 1 to find next-hop entities or possible answers and extract the semantics of $x$ as $sem[x,Q,clues]$, leading to expansion of $\&G$ for further reasoning. A node $x$ should be revisited once acquiring new $clues[x,\&G]$, i.e., when there is a new edge links to it. Finally, a predictor model predicts answer probabilities of candidates based on the final hidden representation $\mathbf{X}$ from System 2.


==> garbage.tex <==
% \textbf{Conditional Ontology Model}. Given a set of topics of relation $T = \{r_1, r_2,...\} \subset R$, build an ontology which only contains and classifies related instances.\\
% \subsection{Hierarchical Graph}
% HG is composed by two part: instance graph and concept graph. \\Instance graph $G_I$ is a general knowledge graph without ontology. $G_0 = (V_I, E_I)$, where each edge $e \in E_I$ represents a piece of $r(e)$ relation. $\forall e \in E_I, r(e) \in \{0,1,...,R-1\}$. 

% concept graph $G_C=(V_C, E_C)$ is a tree. every edge $e = (v_i, v_j) \in E_C$ indicates that concept $v_i$ is a \emph{Subclass\_Of} $v_j$. 

% Finally, there are also a set of edge $E_{IC}$, in which $(v_i, v_j), v_i \in V_I, v_j \in V_C$ means that $v_i$ is an \emph{Instance\_Of}  concept $v_j$. 


% $HG = (V_I + V_C, E_I + E_C + E_{IC})$.

% \subsection{Abstract Generator}
% An Example is usually used for illustrating the limits of deep learning: Human can recognize ``cat'' after barely a glance of a cat but DL models need millions of cat images. The reasons behind it are that human leverages high-level 
% information trained from other categories of images. So, we want a predictor based on all instances belonging to a common high-level concept. 

% $$P(t | h_0, r_0, V_R(h_0,r_0,HG))$$
% where
% \begin{equation*}
% V_R(h, r, HG) =\{e=(v_i, v_j) \in E_I, r(e) = r \ and\\ \exists c \in V_C, c \ is \ ancestor \ of \ both\ h \ and \ v_i\}
% \end{equation*}

% The abstract generator generates instances and relations with a ``Uncertainty''.

% \subsection{Thought graph}
% Thought graph is a small knowledge graph and only containing nodes related to a specific question $(h_0, r_0, ?)$. Each node in thought graph is assigned a ``uncertainty value'' $u(v_i)$. Suppose we have pre-trained embedding for every kind of relation and then GNNs~\cite{battaglia2018relational} are used for reasoning out the final result.

% \subsection{Reasoning paths}
% Train a RNN to predict which relation should be used next!


\subsection{Construction of Cognitive Graph}
Suppose $P(\*x|h, r)$ be the probability of node $x$ occurring in the paths to reasoning (h,r,?). To leverage NNs as generator, embedding of h and r must be used.

% \textcolor{gray}{Let $\*z \sim \mathcal{N}(0,1)$ be latent variable, $P(\*x|h, r)$ can be modeled as $G(\*{emb}_h + \*z, \*{emb}_r)$.}

$P(\*x|h, r)$ can be modeled as $G(\*{emb}_h, \*{emb}_r)$ by hierarchical softmax. Given a batch of $\*z$ from $[0,1]$ uniformly, a batch of nodes $X$ are generated. Next, we will extend $X$ into a subgraph.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{img/BERT-finetuning.png}
    \caption{Generation of Next-Hop Node Using BERT.}
    \label{fig:my_label}
\end{figure*}

For texts, $P(\*x|h, r)$ can be probabilities of positions in sentence to be relevant to the final answer in a BERT, which is fine-tuned according to the loss in section ~\ref{link12}.

\subsection{Generation of Cognitive Graph}\label{link12}
The last part is similar to imagination in human cognition and now we connect them in the mind. 

Previous work about subgraph sampling is related to this problem~\cite{maiya2010sampling}. The key idea is extend \textit{seed nodes} $\{v\}$ with their neighbours into $\mathcal{G}'$. This algorithm should be slightly modified so that $P_\theta(v|h, r)$ of neighbours are considered. 
And we need gradients about \textit{whether it is useful in reasoning} for nodes in $\mathcal{G}'$. Inspired by \textit{policy gradient}\cite{sutton2000policy} in reinforcement learning, we define \textit{Relevance $\&R_v = \frac{\partial L(\*p, t)}{\partial \alpha_v}$} as the reward for action \textit{generating $v$ into $\&G'$}. 
\[J(\theta) = \nabla_\theta\E_{P_\theta(v|h, r)} \&R_v = \E_{P_\theta(v|h, r)} \nabla_\theta \log P_\theta(v|h, r)\&R_v\]
Therefore, the parameters $\theta$ can be updated corresponding to:
\[\theta \gets \theta + lr\cdot \nabla_\theta \log P_\theta(v|h, r)\&R\]
\subsection{Cognitive Graph Net}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/gnn.png}
    \caption{GNN}
    \label{fig:GNN}
\end{figure*}
\textit{Cognitive GraphNet} is a continuously performed GNN(Figure~\ref{fig:GNN}) with a weight parameter $\alpha$ each node for propagation. When $\alpha_x$ is reduced to nearly zero, the node x takes very little effects in model. The gradient of $\alpha$ can serve as loss for generation. 
\begin{algorithm}
\caption{Cognitive GraphNet Propagation}
\KwIn{
    \\
    Cognitive Graph $\&G$ \\
    BERT $\&B$\\
    Question $q$\\
    Wiki Database $\&W$\\
    }
\KwOut{
    \\
    Nodes' probabilities to be target $\*p$\\
    Nodes' relevance to the query $\frac{\partial \&L(\*p, t)}{\partial \alpha_v}$
}
Initialize queue $\&Q=\{s\}$, node features $f_{v_i} = \*0$, edge features $f_{v_i\to v_j}= \*0$\\
$f_s \gets emb_s$\\
\Repeat{Convergence or specified steps}{
    $x \gets \&Q$.pop()\\
    \If{$x \neq s$}{
    $\{\*f_u\}\gets$ features of all edges ($u_i \to x$)\\
    $\*f_x = \alpha_x G(\{\*f_u\}, \*f_x)$\\
    }
    \For{all edges ($x \to y$)}{
        $\*f_{x \to y} \gets F(\*f_x, \*r_{x \to y})$\\
        \If{$y \notin \&Q$}{$\&Q$.push(y)}
    }
    
}
\For{all nodes x}{
$p_x \gets T(\*f_x)$
}
Backprop($\&L(\*p, t))$\\
\textbf{Return}  $\*p$ and $\frac{\partial L(\*p, t)}{\partial \alpha_v}$
\end{algorithm}
% \section{Example}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{WechatIMG17.jpeg}
%     \caption{Example}
%     \label{fig:example}
% \end{figure}

